The Physical Thickness of Stellar Disks to z ~ 2

In local disk galaxies such as our Milky Way, older stars generally inhabit a thicker disk than their younger counterparts. Two competing models have attempted to explain this result: one in which stars first form in thin disks that gradually thicken with time through dynamical heating, and one in which stars form in thick disks at early times and in progressively thinner disks at later times. We use a direct measure of the thicknesses of stellar disks at high redshift to discriminate between these scenarios. Using legacy HST imaging from the CANDELS and GOODS surveys, we measure the rest-optical scale heights of 491 edge-on disk galaxies spanning 0.4 < z < 2.5. We measure a median intrinsic scale height for the full sample of 0.74 +/- 0.03 kpc, with little redshift evolution of both the population median and scatter. The median is consistent with the thick disk of the Milky Way today (0.6 - 1.1 kpc), but is smaller than the median scale height of local disks (~1.5 kpc) which are matched to our high-redshift sample by descendant mass. These findings indicate that (1) while disks as thick as the Milky Way's thick disk were in place at early times, (2) to explain the full disk galaxy population today, the stellar disks in galaxies need to on average physically thicken after formation.

==> additional_text <==
%RESTFRAME WAVELENGTH
%Our measurements of scale height are in observed restframe near-infrared. This band is the best option given the availability of \emph{HST} data and comparisons with SDSS. Our restframe wavelength is near half a micron. This means we are primarily tracing blue light.

Because the majority of our galaxies have $z > 1$, the higher redshift bin is more completely sampled. This manifests as a tight cluster of scale heights spanning 0.6--1.1 kpc. The distribution has a tail of points at higher scale heights, although these are still typically less than 1.5 kpc. In general, galaxy disks at high redshift are thin and show only mild evolution over time.


This indicates that, on average, the stellar disks of galaxies must have thickened at late times (i.e., $z < 0.5$)---which is needed to account for the thicker disks measured today.  This could support thick disk evolution later in the life of galaxies. Figure \ref{fig:scales} shows that the $z > 1$ region is well-sampled, but later galaxies lack a statistically robust sample. We postulate that thick disks likely formed within the last 8 Gyr.

%--the largest Cycle 1 project, surveying half a million galaxies in the mid- and near-infrared--
%These data can be expanded with redder bands, such as those provided with \emph{JWST}. Dust attenuation diminishes at wavelengths greater than 2 microns. With our results using 0.5 microns, even slightly more red filters would mitigate the effects of dust. Further observations in redder bands would also allow for a more representative sampling of stellar masses. This would clarify the trends we see by ensuring the scale heights are not unduly biased toward younger stars.}}

%By observing galaxies in bluer filters, we are tracing primarily younger stars. These stars shine brightly, dominating the light we observe. The stellar mass, however, is dominated by significantly-dimmer low-mass stars. We recognize that this presents a bias and mitigate it by focusing on the evolution of scale height. We track the same stellar population over time to show how scale height changes with redshift. Older stars are redder and generally located in thicker disks than younger stars. We do not expect this to alter our results, but it is an avenue for further exploration.


%When measuring scale heights, we must consider dust. Dust attenuation is a factor at 0.5 $\mu$m, which means the brightness profiles of our galaxies may have dust contamination. 



%,  Instead of a single average scale height for the \emph{HST} Frontier Fields Parallels, the results are divided into redshift bins \citep{2017ApJ...847...14E}. The average scale height at low redshift, defined as $0.5 < z < 1.5$, is 1.03 $\pm$ 0.25 kpc. Combining the low and intermediate redshift bins for our sample (i.e., $0.4 \leq z \leq 1.7$), we measure a median scale height of 0.91 $\pm$ 0.05 kpc---in good agreement with the \citet{2017ApJ...847...14E} low redshift average. 

At intermediate redshift, defined as $1.5 < z < 2.5$, the average scale height is 0.63 $\pm$ 0.24 kpc. 

The median of the scale heights measured in our work, 0.94 $\pm$ 0.04 kpc, agrees well with these previous measurements from \citet{2006ApJ...650..644E, 2017ApJ...847...14E}. 


%Both the measurements from these studies and in this work look at distant galaxies, meaning we are unable to distinguish between the thick and thin disk components. Thus, all measurements of scale height are presented as composite values, strictly calculating the physical thickness of stellar disks.


As is evident in Figure \ref{fig:today}, the Milky Way thick disk is thicker than the thin disks we observe at high redshift.

The thick disk range of estimates, however, encompasses both our average and inclination-corrected scale heights (solid and dashed red lines, respectively). 

%Using the dataset described in \S \ref{sec:data}, we measure the projected vertical scale height for each galaxy in our sample. To do so, we extract $4 \times 4$ arcsec postage stamps of each galaxy in each of the three bands. 
%For a consistent comparison, we want to measure the scale heights at the same rest wavelength for our full galaxy sample. As seen in Figure \ref{fig:rest}, we move from redder to bluer filters as redshift decreases. This rest window spans 0.46-0.66 microns. At this wavelength, we trace starlight while mitigating dust contamination. This range corresponds to the Sloan Digital Sky Survey (SDSS) g-band.

%This presents two main challenges. First, we must convolve the intrinsic model with a one-dimensional function in two-dimensional space. We solve this by applying a kernel. Second, by looking at these high-redshift galaxies, we are close to the resolution limit of \emph{HST}. Sufficiently thin stellar disks may only be slightly thicker than this limit. Comparison with the kernel, however, shows that we do indeed measure small broadening above and beyond the nominal PSF.

%Our prior allows the three variables shown in \ref{eq:sech2} to fluctuate. The amplitude, nominally the highest value in the surface brightness profile, can vary between zero and ten times that amount. The vertical distance from the galaxy midplane can shift from 3 pixels above or below the location of the brightest value in the galaxy's vertical profile. The scale height, our variable of interest, can range from zero to ten pixels, for a range of $\sim$0.6 arcseconds.

%The fitting process fails for some of the galaxies. Out of 527 galaxies, 36 have bad fits. These are characterized by having a scale height of 10 pixels or greater. In such cases, the fitting process bottoms out before finding a suitable scale height. This is overwhelmingly due to contaminants on the postage stamps that were not removed in data cleaning, such as bright spots.

% We obtain a scale height for every column in all \numsample{} galaxies. Figure \ref{fig:corner} shows the combined fits across an entire galaxy as a radial scale height plot. The scatter is $1\sigma$ above and below. The fit is best near the center of the galaxy and becomes less certain at its outskirts. This is due to the low signal to noise ratio farther from the center of the disk. Partially to counter this, we define the average scale height for a galaxy as to be that measured at the effective radius. We take the scale heights of the two columns on either side of the effective radius on both sides of the galaxy. This yields four scale heights at the effective radius. We then take the mean of these as the scale height for the galaxy. The standard deviation of the mean is the uncertainty on this scale height.

%A caveat to the process of finding scale heights is the effect of galaxy inclination. If a galaxy is primarily edge-on yet still tilted with respect to our sightline, its scale height will be artificially enlarged. See Appendix \ref{sec:biases} for a full treatment. We find that the recovered scale height is, on average, 22\% higher than the intrinsic scale height. We present intrinsic results as well as those corrected by this factor.

%In the right panel of Figure \ref{fig:scales}, we show the distribution of the sample, along with the median and corrected median.
%As previously mentioned, we mitigate the effects of galaxy inclination through modeling (see Appendix \ref{sec:biases}). The scale heights shown are those measured from the fitting process. We calculate an average correction factor of 22\% on these measurements. The dashed red lines show the median impact this correction has on the scale heights. 
%Although our measured scale heights have a median of 0.94 kpc, we estimate the true average of the galaxy population to be 0.73 kpc based on inclination corrections.

%As discussed in \S\ref{sec:methods}, we do not consider potential dust obscuration.As seen in Figures \ref{fig:scales} and \ref{fig:today}, we measure predominantly thin disks. If these disks appear artificially inflated by the effects of dust, that only strengthens our conclusion that thin disks were preferential at early times. \citealt{2014ApJ...787...24B} modeled the effects of dust on our SDSS comparison galaxies, so those scale heights in Figure \ref{fig:today} can be taken as accurate to within 15\%.

%When measuring scale heights, we must consider dust. Dust attenuation is a factor at 0.5 $\mu$m, which means the brightness profiles of our galaxies may have dust contamination. Dust tends to line the midplane of galaxies, suppressing light. A dust-obscured galaxy would appear to have a thicker disk than its intrinsic thickness. We would see this in our analysis as a flattened profile. Looking at our data as a whole, we do not see evidence of dust contamination. As seen in Figures \ref{fig:scales} and \ref{fig:today}, we measure predominantly thin disks. If these disks appear artificially inflated by the effects of dust, that only strengthens our conclusion that thin disks were preferential at early times. \citealt{2014ApJ...787...24B} modeled the effects of dust on our SDSS comparison galaxies, so those scale heights in Figure \ref{fig:today} can be taken as accurate to within 15\%.
